Empowering Graph Representation Learning with Test-Time Graph Transformation

As powerful tools for representation learning on graphs, graph neural networks (GNNs) have facilitated various applications from drug discovery to recommender systems. Nevertheless, the effectiveness of GNNs is immensely challenged by issues related to data quality, such as distribution shift, abnormal features and adversarial attacks. Recent efforts have been made on tackling these issues from a modeling perspective which requires additional cost of changing model architectures or re-training model parameters. In this work, we provide a data-centric view to tackle these issues and propose a graph transformation framework named GTrans which adapts and refines graph data at test time to achieve better performance. We provide theoretical analysis on the design of the framework and discuss why adapting graph data works better than adapting the model. Extensive experiments have demonstrated the effectiveness of GTrans on three distinct scenarios for eight benchmark datasets where suboptimal data is presented. Remarkably, GTrans performs the best in most cases with improvements up to 2.8%, 8.2% and 3.8% over the best baselines on three experimental settings. Code is released at https://github.com/ChandlerBang/GTrans.

==> README.tex <==
Defensive Patches for Robust Recognition in the Physical World

MEMO: Test Time Robustness via Adaptation and Augmentation:
Though effective at handling test shifts, these methods sometimes still require specialized training procedures, and they typically rely on extracting information via batches or even entire sets of test inputs, thus introducing additional assumptions.
We are interested in studying and devising methods for im- proving model robustness that are “plug and play”, i.e., they can be readily used with a wide variety of pretrained models and test settings.
we also want methods that synergize with other robustification techniques, in order to achieve greater performance than using either in isolation. 



section 3.4 analysis
https://openreview.net/pdf?id=r8S93OsHWEf



Jundong 
https://dl.acm.org/doi/pdf/10.1145/3485447.3512173

It is costly to fine-tune existing debiasing algorithms for each specific GNN architecture. Different


There are already debiasing approaches modifying original datasets via perturbing data distributions or reweighting the data points in the dataset [8, 25, 57]. These ap- proaches obtain less biased datasets, which help to mitigate bias in learning algorithms. In this regard, considering that debiasing for different GNNs is costly, it is also desired to mitigate the bias in attributed networks before they are fed into GNNs


Taylor expansion\url{https://www.cs.purdue.edu/homes/hmaji/teaching/Spring%202019/lectures/note01.pdf}

==> other_thoughts.tex <==

\wei{Some questions I hope I can answer: (a) when do we need  structure modification and when do we need feature modification?  --> with unlimited perturbation budget, probably feature perturbation is more effective???? --> if the structure is missing, we can learn propagated features; but if the feature is missing, it is impossible to learn features by solely structure? ---> (b) then why is structure learning necessary?? }

\wei{My answer would be: probably feature perturbation is favorable. Here are the reasons. Let’s consider a decoupled GNN architecture (AXW). If the structure A is missing, we can always recover the propagated features by modifying X; but if the feature is missing, it is impossible to recover the propagated features by modifying solely structure as we do not modify X .
Then when is learning structure helpful? For a coupled GNN, say A(AXW)W, when A is missing or corrupted,  to recover the original forward process of GNN, we do need to modify A  since only modifying X does not achieve the goal.}



==> proof2.tex <==
\begin{theorem}
Assume that the augmentation function $\mathcal{A}(\cdot)$ generates a data view of the same class for the test nodes and the node classes are balanced. For each class, the mean of the representations obtained from ${\bf Z}$ and $\hat{\bf Z}$ are the same.
\end{theorem}
\begin{proof}
For convenience, we slightly abuse the notations to replace $\frac{z_i}{\|z_i\|}$ and $\frac{\hat{z}_i}{\|\hat{z}_i\|}$ with $z_i$ and $\hat{z}_i$, respectively. Then we have $\|z_i\|=\|\hat{z}_i\|=1$. Let $Z_k$ denote the set of test samples from class $k$; thus $|Z_k|=\frac{N}{K}$. Let $\stackrel{c}{=}$ denote equality up to a multiplicative and/or additive constant. We start from analyzing the first term in Eq.~(\ref{eq:contrast}), which can be rewritten as 
\begin{equation}
\begin{aligned}
& \sum^N_{i=1} (1-\hat{z}_i^\top_i\hat{z}_i ) = \sum^N_{i=1} \left(\|z_i\|^2 -\hat{z}^\top_i z_i\right)  = \sum^K_{k=1} \sum_{z_i\in Z_k}\left(\|z_i\|^2 -\hat{z}^\top_i {z}_i\right)  \\
\stackrel{c}{=} &   \sum^K_{k=1} \frac{1}{|Z_k|}\sum_{z_i\in Z_k}\left(\|z_i\|^2 -\hat{z}^\top_i {z}_i\right) \\
\stackrel{c}{=} &   \sum^K_{k=1} \frac{1}{|Z_k|}\sum_{z_i\in Z_k} -\hat{z}^\top_i {z}_i
\end{aligned}
\end{equation}
% Since $\|z_i\|=\|\hat{z}_i\|=1$, we have
% \begin{equation}
%     \sum^K_{k=1} \frac{1}{|Z_k|}\sum_{z_i\in Z_k} -\hat{z}^\top_i\hat{z}_i  \stackrel{c}{=} \sum^K_{k=1} \frac{1}{|Z_k|}\sum_{z_i\in Z_k} \left( \|\hat{z}_i\|^2 - \hat{z}^\top_i\hat{z}_i \right) = \sum^K_{k=1} \sum_{z_i\in Z_k} \left( \|\hat{z}_i\|^2 - \hat{z}^\top_i\hat{z}_i \right)
% \end{equation}
Let $c_k$ be the mean of hidden representations from class $k$, i.e., $c_k=\frac{1}{|Z_k|}\sum_{{z}_i\in Z_k}{z}_i$. We replace $\sum_{\hat{z}_i\in Z_k}\|\hat{z}_i-c_k\|^2$. Later,
\begin{equation}
\begin{aligned}
& \sum_{z_i\in Z_k} \|z_i-c_k\|^2= \sum_{z_i\in Z_k} \|z_i\|^2 - 2 \sum_{z_i\in Z_k} z_i^\top c_k + |Z_k|\|c_k\|^2 \\
= & \sum_{z_i\in Z_k} \|z_i\|^2 - 2  \frac{1}{|Z_k|}\sum_{z_i\in Z_k}\sum_{\hat{z}_i\in \hat{Z}_k}\hat{z}^\top_i z_i +  \frac{1}{|Z_k|}\sum_{z_i\in Z_k}\sum_{\hat{z}_i\in \hat{Z}_k}\hat{z}^\top_i z_i \\
= & \sum_{z_i\in Z_k} \|z_i\|^2 - \frac{1}{|Z_k|}\sum_{z_i\in Z_k}\sum_{\hat{z}_i\in Z_k}\hat{z}^\top_i z_i \\
\stackrel{c}{=} & \frac{1}{|Z_k|}\sum_{z_i\in Z_k} \sum_{\hat{z}_i\in \hat{Z}_k} \|z_i\|^2 - \frac{1}{|Z_k|}\sum_{z_i\in Z_k}\sum_{\hat{z}_i\in Z_k}\hat{z}^\top_i z_i \\
= & \frac{1}{|Z_k|}\sum_{z_i\in Z_k} \sum_{\hat{z}_i\in \hat{Z}_k}\left( \|z_i\|^2 - \hat{z}^\top_i z_i \right) \\
\stackrel{c}{=}  & \frac{1}{|Z_k|}\sum_{z_i\in Z_k} \sum_{\hat{z}_i\in \hat{Z}_k}\left( - \hat{z}^\top_i z_i \right)
\end{aligned}
\end{equation}
As we assume $\mathcal{A}(\cdot)$ generates can simulate the test nodes from the same class.
\end{proof}
The proof is based on the work~\citep{boudiaf2020unifying}.

\begin{theorem}
Given a pretrained network $f_\theta$ and test data samples $\{x_i|i=1,\ldots,K\}$,  finetuning the model $f_\theta$ is no more powerful than finetuning the data $\{x_i|i=1,\ldots,K\}$ at test stage.
\end{theorem}
\begin{proof}
Suppose we have two test samples $x_1, x_2$ with corresponding label $y_1$ and $y_2$, respectively, and $y_1$ and $y_2$ belong to the label space of training data. Then we consider the following mean square error:
\begin{equation}
    \ell = (f_\theta(x_1) - y_1)^2 + (f_\theta(x_2) - y_2)^2.
\end{equation}
It is easy to see that $\ell$ reaches its minimum when $f_\theta(x_1)=y_1, f_\theta(x_2)=y_2$.

Suppose the two test samples have the same features but different labels, i.e., $x_1=x_2, y_1\neq y_2$. Note that this scenario is practical when considering adversarial attacks or abnormal features. In this context, it is impossible to find $\theta$ with which $f_\theta$ can map $x_1, x_2$ to different labels since $f_\theta$ is a many-to-one function. However, since $y_1$ and $y_2$ are in the label space of training data, there are two training samples $\hat{x}_1, \hat{x}_2$ such that $f_\theta(\hat{x}_1)=y_1, f_\theta(\hat{x}_2)=y_2$.
Hence, we can always find  by modifying the data samples $x_1, x_2$.

On the other hand, we consider $x_1\neq x_2, y_1\neq y_2$. Whether we can find $\theta$ that satisfies $x_1\neq x_2, y_1\neq y_2$ depends on the expressiveness of the the function $f_\theta$. For example, unlike MLP, some GNNs have limited expressive power~\citep{xu2018powerful,Oono2020Graph}. By contrast, finetuning the data does not suffer this problem as we can possibly modify $x_1$ to $\hat{x}_1$ and $x_2$ to $\hat{x}_2$. 
\end{proof}

==> sections/method_backup.tex <==

\section{Methodology}
\ns{if you have time, maybe we consider breaking this section up a bit.  currently, it contains some notation and problem-related preliminaries as well as methods, but we can perhaps split it up so that we propose a general problem, and then propose our method for solving it.  there could be other methods, but making the problem framing explicit may make it easier for others to reference this work and also work on the more generalized problem of test-time graph transformation.}
We start by introducing the general framework \method{} for test-time graph transformation. Although our discussion mainly focuses on the node classification task where the goal is to predict the labels of nodes in the graph, we note that our framework can be easily extended to other tasks. \tz{if we don't have experiments on other tasks, maybe we should make this clear in the introduction?} \wei{it should be fine. We can just highlight it here.} Consider that we have a training graph $G_\text{Tr}$ and a test graph $G_\text{Te}$, and the corresponding set of node labels are denoted as $\mathcal{Y}_{\text{Tr}}$ and $\mathcal{Y}_{\text{Te}}$, respectively. Note that \textit{we do not have the assumption that the nodes in $G_\text{Tr}$ and $G_\text{Te}$ are drawn from the same distribution}. \ns{do we make any assumptions about the disjointness of the graphs?  can they be overlapping?  either way we should clarify because it currently sounds like the training graph and test graph are totally disjoint.} \wei{the datasets used for experiments have both inductive and transductive setting. The training graph and test graph can either have overlaped nodes or not; but one thing for sure is that these two graphs are not exactly the same (either node features or structure)} Further, let $f_\theta(\cdot)$ denote the mapping function of a GNN model parameterized by $\theta$, which maps a graph into the space of node labels. The core of \method{} is the graph transformation function $g(\cdot)$ which refines the test graph $G_\text{Te}$ such that the pretrained $f_\theta$ can yield better test performance on $g(G_\text{Te})$ than that on $G_\text{Te}$. The process can be expressed as: 
% \begin{equation}
% \begin{aligned}
%     \Delta{G}=\arg \min _{\Delta{G}}  \mathcal{L}& \left(f_{\theta}(G+\Delta{G}), \mathcal{Y}_1\right) \quad \text{with}\;  \theta = \arg \min_{\theta} \mathcal{L}\left(f_{\theta}(G), \mathcal{Y}_2\right) \\
%     & \text{s.t.}\quad \Delta{G} \in \mathcal{P}({G})
% \label{eq:general}
% \end{aligned}
% \end{equation}
\begin{equation}
\begin{aligned}
    \argmin _{g} \mathcal{L}& \left(f_{{\theta}^*}(g(G_{\text{Te}})), \mathcal{Y}_{\text{Te}}\right) \quad \text{s.t.}\quad g({G_{\text{Te}}}) \in \mathcal{P}({G_{\text{Te}}}),  \\
    &  \text{with}\;  \theta^* = \arg \min_{\theta} \mathcal{L}\left(f_{\theta}(G_{\text{Tr}}), \mathcal{Y}_{\text{Tr}}\right),
\label{eq:general}
\end{aligned}
\end{equation}
where $\mathcal{L}$ denotes the classification loss; $\mathcal{P}(G_{\text{Te}})$ is the space of perturbation on the original graph, e.g., we may constrain the change of the graph to be small.
% $g({G_{\text{Te}}})\in\mathcal{P}(G_{\text{Te}})$ indicates that $g({G_{\text{Te}}})$ is chosen from a constrained domain $\mathcal{P}(G_{\text{Te}})$. Specifically, $\mathcal{P}(G_{\text{Te}})$ constrains the . 
To optimize the above formulation, we are faced with two critical challenges: (1) how to parameterize and optimize the graph transformation function $g(\cdot)$ and (2) how to formulate a surrogate loss to guide the learning process, since we do not have access to the ground-truth labels of test nodes. In the following subsections, we elaborate on how \method addresses these challenges.





\subsection{Constructing Graph Transformation}
In this subsection, we introduce how to construct the graph transformation function and detail its optimization process. Let $G_\text{Te}=\{{\bf A}, {\bf X}\}$ denote the test graph, where ${\bf A}\in \{0, 1\}^{N\times N}$ is the adjacency matrix, $N$ is the number of nodes, ${\bf X}\in{\mathbb{R}^{N\times d}}$ is the $d$-dimensional node feature matrix \ns{are there any assumptions on the \# of nodes in the training graph?  i guess it must be less than the test graph. 
we should be explicit about our assumptions for these graphs.}. \wei{We do not have such assumptions; at least in the experiments the test graph can be larger/smaller than the training graph.} Since the pretrained GNN parameters are fixed at test-time, and we only care about the test graph, we drop the subscript in $G_\text{Te}$ and $\mathcal{Y}_\text{Te}$ to simplify notation in the rest of the paper. 


\textbf{Construction.} We are interested in obtaining the transformed test graph
$G'_\text{Te}=g({\bf A}, {\bf X})=({\bf A}', {\bf X}')$. Specifically, we model feature modification as an additive function which injects perturbation to node features, i.e., ${\bf X'}={\bf X}+\Delta{}{\bf X}$; we model the structure modification as ${\bf A}'={\bf A}\oplus\Delta{{\bf A}}$, where $\oplus$ stands for an element-wise exclusive OR operation and $\Delta{{\bf A}}\in \{0,1\}^{N\times N}$ is a binary matrix. In other words,  $\Delta{\bf A}_{ij}=1$ indicates an edge flip.
Formally, we seek to find $\Delta{{\bf A}}$ and $\Delta{{\bf X}}$ that can minimize the objective function:
\begin{equation}
    \argmin _{\Delta{{\bf A}}, \Delta{{\bf X}}}  \mathcal{L} \left(f_{\theta}({\bf A}\oplus\Delta{{\bf A}}, {\bf X}+\Delta{{\bf X}}), \mathcal{Y}\right) \quad \text{s.t.}\quad ({\bf A} \oplus \Delta{{\bf A}}, {\bf X}+\Delta{{\bf X}}) \in \mathcal{P}({{\bf A}, {\bf X}}),
\label{eq:general}
\end{equation}
where $\Delta{{\bf A}}\in \{0,1\}^{N\times N}$ and $\Delta{\bf X}\in{\mathbb{R}^{N\times d}}$ are treated as free parameters. Further, to ensure we do not heavily violate the original graph structure, we constrain the number of changed entries in the  adjacency matrix to be smaller than a budget $B$ on the graph structure, i.e., $\|\Delta{{\bf A}}\|_2\leq B$. We do not impose constraints on the node features to ease optimization. In this context, $\mathcal{P}$ can be viewed as constraining $\Delta{\bf A}$ to a binary space as well as  restricting the number of changes.

\textbf{Optimization.} Jointly optimizing $\Delta{\bf X}$ and $\Delta{\bf A}$ is often challenging as they depend on each other. In practice, we alternatively optimize $\Delta{\bf X}$ and $\Delta{\bf A}$. Notably, the optimization for $\Delta{\bf X}$ is easy since the node features are continuous. The optimization for $\Delta{\bf A}$ is particularly challenging in that (1) $\Delta{\bf A}$  is binary and constrained; and (2) the search space of $N^2$ entries is too large especially when we are learning on large-scale graphs.

To cope with the first challenge, we relax the binary space to $[0,1]^{N\times N}$ and then we can employ projected gradient descent (PGD)~\citep{xu2019topology-attack,geisler2021robustness} to update $\Delta{\bf A}$:
\begin{equation}
\Delta\mathbf{A}\leftarrow{} \Pi_{\mathcal{P}}\left(\Delta\mathbf{A}-\eta \nabla_{\Delta{\bf A}}\mathcal{L}(\Delta{\bf A}) \right)
\end{equation}
where we first perform gradient descent with step size $\eta$ and call a projection $\Pi_{\mathcal{P}}$ to project the variable to the space $\mathcal{P}$. Specifically, given an input vector ${\bf p}$, $\Pi_{\mathcal{P}}(\cdot)$ is expressed as: 
\begin{equation}
\Pi_{\mathcal{P}}({\bf p})\leftarrow{}\left\{\begin{array}{ll}
\Pi_{[0,1]}({\bf p}), & \text { If } \mathbf{1}^{\top} \Pi_{[0,1]}({\bf p}) \leq B; \\
\Pi_{[0,1]}({\bf p}-\gamma \mathbf{1}) \text { with } \mathbf{1}^{\top} \Pi_{[0,1]}({\bf p}-\gamma \mathbf{1})=B, & \text { otherwise, }
\end{array}\right.
\end{equation}
where $\Pi_{[0.1]}(\cdot)$ clamps the input values to $[0,1]$ and $\gamma$ is obtained by solving the equation $\mathbf{1}^{\top} \Pi_{[0,1]}({\bf p}-\gamma \mathbf{1})=B$ with the bisection method~\citep{liu2015sparsity}.
After that, we view each entry in ${\bf A}\oplus\Delta{\bf A}$ as a Bernoulli distribution and sample a discrete graph ${\bf A}' \sim \operatorname{Bernoulli}({\bf A}\oplus\Delta{\bf A})$. 
\ns{this seems a bit confusing.  earlier you define $\Delta\mathbf{A}$ in $\{0,1\}^{N \times N}$. if it is indeed so, then $\mathbf{A} + \Delta\mathbf{A}$ will be defined on $\{0,1,2\}^{N \times N}$ on which this bernoulli sampling doesn't really make sense.} \ns{we should mention why we do this bernoulli sampling.  is it to keep the graph discrete and sparse? the reader would be thinking that this would make the gradients noisy, and probably choosing not to sample would be more stable} \wei{there was a typo about the symbol $+$; it should be $\oplus$}

% To cope with the budget constraints, we follow~\citet{xu2019adversarial} to use a bisection method~\citep{liu2015sparsity}.



Furthermore, to enable efficient graph structure learning, it is desired to reduce the search space of updated adjacency matrix. One recent approach of graph adversarial attack~\citep{geisler2021robustness} proposes to sample a small block of possible entries from the adjacency matrix and update them at each iteration. This solution is still computationally intensive as it requires hundreds of steps to achieve a good performance.
Instead, we constrain the search space to only the existing edges of the graph, which is typically sparse. Empirically, we observe that this simpler strategy still learns useful structure information when combined with feature modification.



\subsection{Parameter-Free Surrogate Loss}
As discussed earlier, the proposed framework \method{} aims to improve the model generalization and robustness by learning to transform the test graph. 
Ideally, when we have test ground-truth labels, the problem can be readily solved by adapting the graph that results in the minimum cross entropy loss on test samples. However, as we do not have such information at test-time, it motivates us to investigate feasible surrogate losses to guide the graph transformation process. In the absence of labeled data, recently emerging self-supervised learning techniques~\citep{xie2021self-survey,liu2022graph} have paved the way for providing self-supervision for test-time graph transformation. However, not every surrogate self-supervised task and loss is suitable for our transformation process, as some tasks are more powerful and some are weaker. To choose a suitable surrogate loss, we provide the following theorem.

%unlabeled data by constructing pretext tasks based on structural and attribute information. The intuition behind SOAP is that the shift in representation z that hinders classification will hinder the auxiliary self-supervised task as well. In


\begin{theorem} Let $\mathcal{L}_c$ denote the classification loss and $\mathcal{L}_s$ denote the surrogate, respectively. Let $\rho(G)$ denote the correlation between $\nabla_{G}\mathcal{L}_c(G,\mathcal{Y})$ and $\nabla_{G}\mathcal{L}_s(G)$, and let $\epsilon$ denote the learning rate for gradient descent. Assume that $\mathcal{L}_c$ is twice-differentiable and its Hessian matrix satisfies $\|H(G, \mathcal{Y})\|_2\leq M$  for all $G$. When $\rho(G)>0$ and $\epsilon < \frac{2\rho\left({G}\right)\left\|\nabla_{{G}} \mathcal{L}_{c}\left({G}, \mathcal{Y}\right)\right\|_{2}}{M\left\|\nabla_{{G}} \mathcal{L}_{s}\left({G}\right)\right\|_{2}}$, we have
\begin{equation}
\mathcal{L}_{c}\left({G}-\epsilon \nabla_{{G}} \mathcal{L}_{s}\left({G}\right), \mathcal{Y}\right) < \mathcal{L}_{c}\left({G}, \mathcal{Y}\right).
\end{equation}
\end{theorem}

The proof can be found in Appendix~\ref{app:thereom1}. Theorem 1 suggests that when the gradients from classification loss and surrogate loss have positive correlation, i.e., $\rho\left({G}\right)>0$, we can update the test graph by performing gradient descent with a sufficiently small learning rate such that the classification loss on the test samples is reduced. Hence, it is important to find a surrogate task that shares relevant information with the classification task. 

%Graph contrastive learning broadly follow a contrasting scheme, where the similarity between two augmented views from the same sample is maximized while the similarity between views from two different samples is minimized.

\textbf{Parameter-Free Surrogate Loss.} As one popular self-supervised paradigm, graph contrastive learning has achieved promising performance in various graph-related  tasks~\citep{hassani2020contrastive,you2021graph,zhu2021graph}, which indicates that graph contrastive learning tasks are often highly correlated with downstream tasks.  This property is desirable for guiding test-time graph transformation as suggested by Theorem~1. At its core lies the contrasting scheme, where the similarity between two augmented views from the same sample is maximized, while the similarity between views from two different samples is minimized. 

However, existing graph contrastive learning methods cannot be directly applied to our scenario, as they requires a parameterized projection head to map augmented representations to another latent space, which inevitably alters the model architecture. 
To address this issue, we propose a parameter-free surrogate loss. Specifically,
we apply an augmentation function $\mathcal{A}(\cdot)$ on input graph $G$ and obtain an augmented graph $\mathcal{A}(G)$. The node representations obtained from the two graphs are denoted as $Z$ and $\hat{Z}$, respectively; ${\bf z}_i$ 
and $\hat{\bf z}_i$ stand for the $i$-th node representation taken from $Z$ and $\hat{Z}$, respectively. Essentially, we maximize the cosine similarity between original nodes and their augmented view while penalizing the similarity between the nodes and their negative samples:
\begin{equation}
    \min \mathcal{L}_s = \sum_{i=1}^{N} (1-\frac{\hat{\bf z}_i^\top {\bf z}_i}{\|\hat{\bf z}_i\|\|{\bf z}_i\|}) - \sum_{i=1}^{N} (1-\frac{\tilde{\bf z}_i^\top {\bf z}_i}{\|\tilde{\bf z}_i\|\|{\bf z}_i\|}),
\label{eq:contrast}
\end{equation}
% \begin{equation}
%     \arg\min \sum_{({\bf z}_i, \hat{\bf z}_i)\in\mathcal{X}^p} (1-\frac{\hat{\bf z}_i^\top {\bf z}_i}{\|\hat{\bf z}_i\|\|{\bf z}_i\|}) - \sum_{({\bf z}_i, \tilde{\bf z}_i)\in\mathcal{X}^n} (1-\frac{\tilde{\bf z}_i^\top {\bf z}_i}{\|\tilde{\bf z}_i\|\|{\bf z}_i\|})
% \label{eq:contrast}
% \end{equation}
where $\{\tilde{\bf z}_i|i=1,\ldots,N\}$ are the  negative samples for corresponding nodes, which are generated by shuffling node features~\citep{velickovic2019deep}. Remarkably, the hidden presentations ${\bf z}_i, \hat{{\bf z}}_i, \tilde{{\bf z}}_i$ are directly taken from the output of the second last layer of the pretrained model. In Eq.~(\ref{eq:contrast}), the first term encourages each node to be close to 
while second term pushes each node away from the corresponding negative sample. 

We note that the above surrogate loss have two compelling advantages: (1) it is parameter-free, and does not require modification of the model architecture, or affect the pretraining process; and (2) we only have one augmented view instead of two, which eases the analysis in Theorem 2 \ns{perhaps we should not mention this easing of the analysis when we haven't introduced thm 2 yet; seems a little confusing}.  Furthermore, we also empirically compare the proposed surrogate loss with other self-supervised signals in Section~\ref{sec:ssl}.


%\textbf{Complexity Analysis.}

% $\rho\left({G}\right)\left\|\nabla_{{G}} \mathcal{L}_{c}\left({G}, \mathcal{Y}\right)\right\|_{2}\left\|\nabla_{{G}} \mathcal{L}_{s}\left({G}\right)\right\|_{2}$ is large, the classification loss will reduce.

\iffalse
\subsection{Applications}
% \textbf{Cold-start problem.} When a GNN model is deployed in a recommender system, it is hard to accurately predict the preference of a new user  as the user’s past behavior is very limited, which is often referred as the cold-start problem. With the aforementioned general framework, we can learn to modify the graph structure of the user-item interaction graph so as to improve the performance on those new users. For example, we plan to model $\mathcal{Y}_1$ as the user nodes with lower degrees and $\mathcal{Y}_2$ as the nodes with higher degrees. \wei{can entropy minization with structure perturbation help?}

% \textbf{Noisy graphs and non-homophily graphs.} When the graph contains noise or the graph does not follow the homophily assumption, GNNs tend to yield less promising performance~\citep{zhu2020beyond}. To promote their performance on such graphs, a natural solution is to modify the graph that better fits GNNs' ability. We plan to model $\mathcal{Y}_1$ and $\mathcal{Y}_2$ as two different training sets of node labels for the node classification task.

\textbf{Distribution shift.} As observed in~\citep{zhu2021shift,wu2022handling}, 
the bias in the sampling process to select nodes for training can cause distributional differences between the training set and the rest of the graph. GNNs can suffer poor generalization when the distribution shift occurs. Our framework is able to learn a graph perturbation to transform the graph structure which involves both training nodes and test nodes. We plan to use a domain invariant loss in the outer optimization of Eq.~\eqref{eq:general} and a cross-entropy classification loss in the inner optimization. \wei{similar to test-time training, we can use ssl loss as the test-time loss to update the graph..}

% \textbf{Fairness.} When sensitive information is contained in the node features, GNNs can produce severe bias in decision making, i.e., the predictions are highly correlated with the sensitive attributes of the nodes~\citep{dai2021say}.  The bias would largely limit the wide adoption of GNNs in domains such as ranking of job applicant. We plan to include some fairness constraint in the outer optimization of Eq.~\eqref{eq:general} to make the predictions invariant with the estimated sensitive attributes.


% \textbf{Privacy.}
\fi



\subsection{Further Analysis}\label{sec:analysis}
In this subsection, we study the theoretical property of the proposed surrogate loss and compare the strategy of adapting data versus that of adapting model. We first demonstrate the rationality of the proposed surrogate loss through the following theorem. 

\begin{theorem}
Assume that the augmentation function $\mathcal{A}(\cdot)$ generates a data view of the same class for the test nodes and the node classes are balanced. Assume for each class, the mean of the representations obtained from ${Z}$ and $\hat{Z}$ are the same. Minimizing the first term in Eq.~(\ref{eq:contrast}) is approximately minimizing the class-conditional entropy $H({ Z}|{Y})$ between features $Z$ and labels $Y$.
\end{theorem}

The proof can be found in Appendix~\ref{app:thereom2}. Theorem 2 indicates that minimizing the first term in Eq.~(\ref{eq:contrast}) will minimize $H(Z|Y)$, which encourages high intra-class compactness, i.e., learning a low-entropy cluster in the embedded space for each class. However, we note that using this term only can result in collapse (mapping all data points to a single point in the embedded space), which indicates the necessity of the second term in Eq.~(\ref{eq:contrast}).

Next, we use an illustrative example to show that adapting data at test-time can be more useful than adapting model in some cases. \wei{still working on it..}

\textbf{Example.} Given test data samples $\{{\bf x}_i|i=1,\ldots,K\}$, we consider a linearized GNN $f_\theta$ which first performs aggregation through a function $\text{Agg}(\cdot,\cdot)$ and then transform the aggregated features via a function $\text{Trans}(\cdot)$. If there exist two nodes with the same aggreagated features but different labels, i.e., $\text{Agg}({\bf x}_1, \{{\bf x}_i|i\in \mathcal{N}_{1}\})=\text{Agg}({\bf x}_2, \{{\bf x}_j|j\in \mathcal{N}_{2}\}), y_1\neq{y_2}$, adapting the data $\{{\bf x}_i|i=1,\ldots,K\}$ achieves lower classification error than adapting the model $f_\theta$ at test stage.


%\textbf{Example.} Given a pretrained network $f_\theta$ and test data samples $\{x_i|i=1,\ldots,K\}$, adapting the data $\{x_i|i=1,\ldots,K\}$ could achieve lower classification error than adapting the model $f_\theta$ at test stage when there exist two data points with ${\bf x}_1={\bf x}_2, y_1\neq{y_2}$.
% \label{prop:1}

\textit{Illustration.}
Suppose we have two test samples ${\bf x}_1, {\bf x}_2$ with corresponding label $y_1$ and $y_2$, respectively, and $y_1$ and $y_2$ belong to the label space of training data. Then we consider the following mean square error:
\begin{equation}
    \ell = \frac{1}{2}\left((f_\theta({\bf x}_1) - y_1)^2 + (f_\theta({\bf x}_2) - y_2)^2\right).
\end{equation}
It is easy to see that $\ell$ reaches its minimum when $f_\theta({\bf x}_1)=y_1, f_\theta({\bf x}_2)=y_2$.

Suppose the two test samples have the same features but different labels, i.e., ${\bf x}_1={\bf x}_2, y_1\neq y_2$. Note that this scenario is practical when considering adversarial attacks or abnormal features. In this context, it is impossible to find $\theta$ such that $f_\theta$ can map ${\bf x}_1, {\bf x}_2$ to different labels since $f_\theta$ is a many-to-one function. However, since $y_1$ and $y_2$ are in the label space of training data, there are two training samples $\hat{\bf x}_1, \hat{\bf x}_2$ such that $f_\theta(\hat{\bf x}_1)=y_1, f_\theta(\hat{\bf x}_2)=y_2$.
Hence, we can always minimize the loss by modifying the data samples ${\bf x}_1, {\bf x}_2$.

On the other hand, we consider ${\bf x}_1\neq {\bf x}_2, y_1\neq y_2$. Whether we can find $\theta$ satisfying ${\bf x}_1\neq {\bf x}_2, y_1\neq y_2$ depends on the expressiveness of the the function $f_\theta$, i.e., the ability to map different data points to different representations/labels. For example, unlike MLP, some GNNs have limited expressive power~\citep{xu2018powerful,Oono2020Graph} and fail to discriminate different samples. By contrast, adapting the data does not suffer this problem as we can possibly modify ${\bf x}_1$ to $\hat{\bf x}_1$ and ${\bf x}_2$ to $\hat{\bf x}_2$. 



% \wei{can we built some connection to transformer and WL test? Expressiveness of graph transformer...(node level) }

% \wei{relationship to test-time data augmentation?...regularization.. we'll see}

